Consistency of the Full and Reduced Order Models for Evolve-Filter-Relax Regularization of Convection-Dominated, Marginally-Resolved Flows

Numerical stabilization is often used to eliminate (alleviate) the spurious oscillations generally produced by full order models (FOMs) in under-resolved or marginally-resolved simulations of convection-dominated flows. In this paper we investigate the role of numerical stabilization in reduced order models (ROMs) of convection-dominated, marginally-resolved flows. Specifically, we investigate the FOM-ROM consistency, i.e., whether the numerical stabilization is beneficial both at the FOM and the ROM level. As a numerical stabilization strategy, we focus on the evolve-filter-relax (EFR) regularization algorithm, which centers around spatial filtering. To investigate the FOM-ROM consistency, we consider two ROM strategies: (i) the EFR-ROM, in which the EFR stabilization is used at the FOM level, but not at the ROM level; and (ii) the EFR-EFRROM, in which the EFR stabilization is used both at the FOM and at the ROM level. We compare the EFR-ROM with the EFR-EFRROM in the numerical simulation of a 2D flow past a circular cylinder in the convection-dominated, marginally-resolved regime. We also perform model reduction with respect to both time and Reynolds number. Our numerical investigation shows that the EFR-EFRROM is more accurate than the EFR-ROM, which suggests that FOM-ROM consistency is beneficial in convection-dominated, marginally-resolved flows.

==> sections/comments.tex <==
\textbf{Experiment 2}
\TI{
My conclusions/comments/questions for Experiment 2 are the following:\\
(1) This is the first time {\it relaxation} is used in the EFR-ROM setting.
Is that correct?
If so, we should explicitly state this in the intro (and abstract?), because it's important to emphasize the {\it novelty} of the paper.}
\\

\maria{Investigating the literature we found https://epubs.siam.org/doi/pdf/10.1137/18M1221618, where the filter is also performed online. I will go trough the draft and correct the statement, and cite the paper.}
\TI{OK :-)}
\\

\TI{
(2) We say that, when $\chi=0.002$, "the systems display oscillatory behavior."
As we discussed during the meeting, could you please add some details about this oscillatory behavior?
Which ROMs are oscillatory: EFR-ROM, EFR-EFRROM, or both?
Are these oscillations spatial or temporal? }
\\

\maria{"Oscillatory behavior" might be misleading... Indeed, in this case, we are talking about the behaviour (vortexes) of the velocity field and of the $C_L$ coefficient.}\\

\TI{
(3) Why do we need $r=50$ instead of $r=3$? \\
(4) Why do we need to take so many snapshots (i.e., $2000$)?}
\\

\maria{
Our first attempt consisted in $200$ snapshots and 20, but it resulted in a poor approximation for $t>4$. We increased the bases number, without solving the problem. We guess that, in order to recover the vortex shedding starting from $t=4$ more information must be collected. This led us to use more snapshots, precisely 2000. The value $r=47$ was chosen in order to retain the $99.9\%$ of the energy of the system. However, once again, we were not able to recover the second half of the velocity field. We tried to overcome these issues with Experiment 3.
}

\textbf{Experiment 3}



\TI{
My conclusions/comments/questions for Experiment 3 are the following:\\
(1) Why does replacing the time interval $[0,8]$ in Experiment 2 with the time interval $[4,8]$ in Experiment 3 work?
What's the reason for the improved results in Experiment 3?
Is it the location of the time interval or the length of the time interval?
In other words, what happens if we replace $[4,8]$ with $[4,12]$?
}\\

\maria{Splitting the interval helps a lot to recover the behaviour for $t>4$. Indeed, concentrate the snapshots information only in that temporal window captures the vortex shedding features. It is not a matter of length of time interval, but of field features. We think that if in $[4, 12]$ we have a comparable vortex dynamic, 2000 snapshots over $[4,12]$ should work. The main problem is that in $[0,4]$ the flux is attached while you can observe a totally different behaviour (vortex shedding) for $t>4$. }
\TI{OK, I see.  I think we should add a sentence or two about this to clarify why we're doing what we're doing.}\\


\TI{Please find below my first comments and questions.}

\subsection{Comments}

\begin{enumerate}
	\item What happens if we do not use EFR at all?
	That is, what happens for the standard G-ROM?
	\TI{Have we addressed this?}
    \item Are we really considering a convection-dominated regime?
\end{enumerate}		

\subsection{Questions}

\begin{enumerate} \itemsep5pt
    \item Journal?  IJNMF?  IJNME?  CMAME? SISC?
    \TI{Try CMAME first.  If it doesn't work, we try IJNME.}
    \item Timeline? 3 months.
	\item Do we observe any {\it oscillations} in our numerical tests?
\end{enumerate}		


\subsection{Next Steps?}

\begin{enumerate} \itemsep10pt

    \item {\bf Sensitivity wrt $\delta$}: \ 
    I think that a sensitivity study of $\delta$ has not been performed in the current literature.  I think that such a study is desperately needed.
    Here are some questions: \\[-0.3cm]
    \begin{enumerate} \itemsep5pt
        \item What is the FE meshsize, $h$?  
        How does $\delta$ compare with $h$?  
        Is it larger?
        \item Is $h$ varying?  
        Is it smaller near the cylinder?  
        If so, I think we should also investigate a \underline{\it variable $\delta$}.  
        That would be original.  
        We chould choose something like $\delta \approx h$ or $\delta \approx 2h$, like people do in LES.
        I think that using variable $\delta$ can improve the results.
    \end{enumerate}		

    \item {\bf Differential Filter (DF)}: \ 
        In Section 4.3 of \cite{xie2017approximate}, two DF types were considered:
        (i) the ROM-DF (Section 4.3.1), which is the ROM version ; and 
        (ii) the FE-DF (Section 4.3.2), which is the FE version.
        Which one are we using?
    

    \item {\bf Higher-Order Differential Filter (HODF)}: \ 
        How about trying the ${\it higher-order}$ DF (HODF) that were proposed in Section 4.1.2 in \cite{gunzburger2019evolve}, but were not carefully investigated? 
        
        To enforce a sharper decay of the DF transfer function, the first type of HODF applies repeatedly the DF filter
        \begin{eqnarray}
	        \left( \bM_r + \delta^2 \, \bS_r \right)^{m} \, \overline{\ba}
	        = \ba \, ,
	        \label{eqn:hodf-1}
        \end{eqnarray}
        where $m$ is the order of the HODF, $\bM_r \in \R^{r \times r}$ is the ROM mass matrix with entries $(\bM_r)_{i j} = ( \bphi_j , \bphi_i)$, $\bS_r \in \R^{r \times r}$ is the ROM stiffness matrix, with entries $(\bS_r)_{i j} = (\nabla \bphi_j , \nabla \bphi_i)$, and $\overline{\ba} \in \R^{r}$ and $\ba \in \R^{r}$ are the vectors of ROM coefficients of the filtered and unfiltered variables $\obu$ and $\bu$, respectively.
 
        The second type of HODF replaces the Laplacian $\Delta$ in the standard DF with an $m$-th order Laplacian, $\Delta^{m}$,  
        \begin{eqnarray}
	        \left( \bM_r + \delta^2 \, \bS_r^{m} \right) \, \overline{\ba}
	        = \ba \, .
	        \label{eqn:hodf-2}
        \end{eqnarray}
        The HODFs are extremely cheap in a ROM setting.  
        This is in contrast to the SEM setting in  \cite{fischer2001filter,mullen1999filtering}, where the HODF is very expensive.  

    \item {\bf Anisotropic DF}: \ 
        We can also propose an anisotropic DF in which we use {\it different ROM lengthscales} (i.e., $\delta_{x}, \delta_{y}, \delta_{z}$) for the three coordinates in the DF.
        This new anisotropic DF is appropriate for the structure-dominated, anisotropic flows that we target.
        (This anisotropic DF seems to require the use of the FE-DF version.)

    \item {\bf FOM-ROM Consistency}: \ 
        One of the main conclusions of this study is that FOM-ROM consistency improves the ROM accuracy.  
        I know that Gianluigi's group has worked on this in the past, and so did we in our group.  
        I think that this FOM-ROM consistency (which has been also called ``model consistency" in the past) is not that well known in the ROM community.  
        So I think that we should add a short discussion.  
        Maybe also look more into it?  
        For example, is the model consistency (i.e., using EFR  both at a FOM and at a ROM level) the only factor?  
        Or should we also look at the ``parameter consistency", i.e., the same $\delta$ values at the FOM and ROM levels?  
        I think that these are all relevant questions.

\item {\bf 3D Tests}: \
What are our options here?  
3D flow past a circular cylinder?
I think that, if possible, we should run a 3D test, since this would increase the paper's value.

\end{enumerate}

